HyperSPNs: Compact and Expressive Probabilistic Circuits

Probabilistic circuits (PCs) are a family of generative models which allows for the computation of exact likelihoods and marginals of its probability distributions. PCs are both expressive and tractable, and serve as popular choices for discrete density estimation tasks. However, large PCs are susceptible to overfitting, and only a few regularization strategies (e.g., dropout, weight-decay) have been explored. We propose HyperSPNs: a new paradigm of generating the mixture weights of large PCs using a small-scale neural network. Our framework can be viewed as a soft weight-sharing strategy, which combines the greater expressiveness of large models with the better generalization and memory-footprint properties of small models. We show the merits of our regularization strategy on two state-of-the-art PC families introduced in recent literature -- RAT-SPNs and EiNETs -- and demonstrate generalization improvements in both models on a suite of density estimation benchmarks in both discrete and continuous domains.

==> tikzlibraryspn.code.tex <==
\usetikzlibrary{chains}
%\usetikzlibrary{arrows}
\usepackage{pgfplots}

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

\pgfmathdeclarefunction{gauss}{2}{%
  \pgfmathparse{1/(#2*sqrt(2*pi))*exp(-((x-#1)^2)/(2*#2^2))}%
}

% int node style
\tikzstyle{int} = [circle,fill=white,draw=black,inner sep=0pt,line width=0.6pt,
minimum size=16pt]


% sum node style
\tikzstyle{sum} = [circle,fill=white,draw=black,inner sep=0pt,line width=0.6pt,
minimum size=16pt, path picture={\draw [shorten >=3pt,shorten <=3pt] (path picture bounding box.south) -- (path picture bounding box.north); \draw [shorten >=3pt,shorten <=3pt] (path picture bounding box.west) -- (path picture bounding box.east);}, node distance=1]

% product node style
\tikzstyle{prod} = [circle,fill=white,draw=black,inner sep=0pt,line width=0.6pt,
minimum size=16pt, path picture={\draw [shorten >=6pt,shorten <=6pt] (path picture bounding box.south east) -- (path picture bounding box.north west); \draw [shorten >=6pt,shorten <=6pt] (path picture bounding box.south west) -- (path picture bounding box.north east);}, node distance=1]

% \intnode [tikz-options] {int node name} 
\newcommand{\intnode}[2][]{
  \node[int, #1] (#2) {$\int$};
}

% \sumnode [tikz-options] {sum node name} 
\newcommand{\sumnode}[2][]{
  \node[sum, #1] (#2) {};
}

% \prodnode [tikz-options] {product node name} 
\newcommand{\prodnode}[2][]{
  \node[prod, #1] (#2) {$\times$};
}
\newcommand{\wprodnode}[3][]{
  \node[prod, #1] (#2) {$\color{#3}\times$};
}

% \maxnode [tikz-options] {max node name} 
\newcommand{\maxnode}[2][]{
  \node[circle,fill=white,draw=black,inner sep=0pt,line width=0.6pt,
  minimum size=16pt, node distance=1, #1] (#2) {\scriptsize $max$};
}

% \emptynode [tikz-options] {generic node name}
\newcommand{\emptynode}[2][]{
  \node[circle,fill=white,draw=black,inner sep=0pt,line width=0.6pt,
  minimum size=16pt, node distance=1, #1] (#2) {};
}

\newcommand{\varnode}[3][]{
  \node[circle,fill=white,draw=black,inner sep=0pt,line width=0.6pt, minimum size=16pt, font=\small, #1] (#2) {#3};
}

\newcommand{\varsqnode}[4][]{
  \node[rectangle, rounded corners=3pt,fill=white,draw=#4,inner sep=0pt,line width=0.6pt, minimum size=19pt, #1] (#2) {#3};
}

\newcommand{\evnode}[4][]{
  \node[circle,fill=#4,text=white,inner sep=0pt, minimum size=16pt, #1] (#2) {#3};
}

\newcommand{\evnodevar}[5][]{
  \node[circle,fill=#4,text=white,inner sep=0pt, minimum size=16pt,
  #1] (#2) {#3};
  \node[below=1pt of #2, xshift=1pt] (#2_vn) {#5};
}

\newcommand{\bernode}[3][]{
  \node[circle,fill=white,draw=black,inner sep=0pt,line width=0.6pt,
  minimum size=16pt, #1] (#2) {\tikz\draw circle (3pt);};
  \node[below=1pt of #2, xshift=1pt] (#2_vn) {#3};
}

\newcommand{\contnode}[3][]{
  \node[circle,fill=white,draw=black,inner sep=0pt,line width=0.6pt,
  minimum size=16pt, node distance=1, #1] (#2) {           
          \begin{tikzpicture} %these distributions look really distorted, and are the ones I want to include, inside the minipage
                \begin{axis}[
                no markers, scale only axis, domain=-4:4,samples=50, smooth,
                axis lines=none,
                height=10pt]
                \addplot [mark=none] {gauss(0,1)};
                \end{axis}
            \end{tikzpicture}};
  \node[below=1pt of #2, xshift=1pt] (#2_vn) {#3};
}

\newcommand{\catnode}[3][]{
  \node[circle,fill=white,draw=black,inner sep=0pt,line width=0.6pt,
  minimum size=16pt, node distance=1, #1] (#2) {           
          \begin{tikzpicture} %these distributions look really distorted, and are the ones I want to include, inside the minipage
                \begin{axis}[
                no markers, scale only axis, domain=-4:4, smooth,
                axis lines=none,
                height=10pt]
                \addplot [mark=none] coordinates { (0,0) (0,10)};
                \addplot [mark=none] coordinates { (-1,0) (-1,7)};
                \addplot [mark=none] coordinates { (-2,0) (-2,3)};
                \addplot [mark=none] coordinates { (1,0) (1,5)};
                \addplot [mark=none] coordinates { (2,0) (2,8)};
                \end{axis}
            \end{tikzpicture}};
  \node[below=1pt of #2] (#2_vn) {#3};
}


% \edge [options] {inputs} {outputs}
\newcommand{\edge}[3][]{ %
  % Connect all nodes #2 to all nodes #3.
  \foreach \x in {#2} { %
    \foreach \y in {#3} { %
      \path (\x) edge [-,line width=0.6pt,#1] (\y) ;%
    } ;
  } ;
}

\newcommand{\upedge}[3][]{
  \path (#2) edge [line width=1pt,->,>=stealth,#1] (#3);
}

\newcommand{\ledge}[4][]{
  \path (#2) edge [line width=1pt,->,>=stealth,#1,edge label=#4] (#3);
}

\newcommand{\weigedge}[4][]{
  \draw[line width=0.6pt,-,#1] (#2) edge node [midway,line width=0.6pt,#1] {#4} (#3) ;
}




%%% Local Variables:
%%% mode: latex
%%% TeX-master: t
%%% End:

